On the Out-Of-Distribution Generalization of Multimodal Large Language Models

We investigate the generalization boundaries of current Multimodal Large Language Models (MLLMs) via comprehensive evaluation under out-of-distribution scenarios and domain-specific tasks. We evaluate their zero-shot generalization across synthetic images, real-world distributional shifts, and specialized datasets like medical and molecular imagery. Empirical results indicate that MLLMs struggle with generalization beyond common training domains, limiting their direct application without adaptation. To understand the cause of unreliable performance, we analyze three hypotheses: semantic misinterpretation, visual feature extraction insufficiency, and mapping deficiency. Results identify mapping deficiency as the primary hurdle. To address this problem, we show that in-context learning (ICL) can significantly enhance MLLMs' generalization, opening new avenues for overcoming generalization barriers. We further explore the robustness of ICL under distribution shifts and show its vulnerability to domain shifts, label shifts, and spurious correlation shifts between in-context examples and test data.

==> paragraphs/acknowledgments.tex <==
\section*{Acknowledgments}


==> paragraphs/app-icl.tex <==
\section{In-context Learning Generalization}
\label{sec:app-icl}

\subsection{ICL with Data from Target Distribution}
Here we show the whole results of GPT-4V and Gemini after ICL with Data from Target Distributions in Table \ref{tab:app-icl-1}.

\begin{table}[th]
\centering
% \begin{subtable}{1.\linewidth}
\caption{Results of ICL with data from target distribution.}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
& XCOVFour & iWildCam & NIH-Chest & CT-XCOV & DrugOOD\_Protein & DrugOOD\_Size & DrugOOD\_Assay & Camelyon17 & HAM10000 \\ 

\midrule
\multirow{4}{*}{\rotatebox{90}{GPT-4V}} & 0.449 & 0.634 & 0.692 & 0.443 & 0.459 & 0.282 & 0.447 & 0.484 & 0.539 \\
& 0.777 & 0.780 & 0.686 & 0.516 & 0.468 & 0.157 & 0.139 & 0.474 & 0.663 \\
& 0.929 & 0.923 & 0.727 & 0.547 & 0.468 & 0.247 & 0.253 & 0.574 & 0.730\\
& 0.917 & 1.000 & 0.751 & 0.438 & 0.468 & 0.287 & 0.272 &  0.536 & 0.742 \\


 \midrule
 \multirow{4}{*}{\rotatebox{90}{Gemini}}& 0.740 & 0.925 & 0.535 & 0.505 & 0.496 & 0.557 & 0.503 & 0.516 & 0.540 \\
& 0.923 & 0.946 & 0.627 & 0.495 & 0.560 & 0.467 & 0.396 & 0.516 & 0.589 \\
& 0.839 & 0.989 & 0.645 & 0.797 & 0.568 & 0.495 & 0.437 & 0.537 & 0.678 \\
& 0.828 & 0.989 & 0.680 & 0.790 & 0.579 & 0.489 & 0.453 & 0.515 & 0.722 \\

\bottomrule
\end{tabular}
}
% \end{subtable}%
\label{tab:app-icl-1}
\end{table}


\subsection{ICL with Spurious Correlation Shifts}
\paragraph{Ommited details of experimental design}
Specifically, we leverage datasets containing two distinct domains ($D_1$ and $D_2$) and two categories ($C_1$ and $C_2$). For ICE, we deliberately craft examples with contrasting domain-category combinations: $C_1$ data from $D_1$ and $C_2$ data from $D_2$. Conversely, test samples mirror the opposite scenario, presenting $C_2$ data from $D_1$ and $C_1$ data from $D_2$. This controlled setting ensures that ICE and test samples exhibit opposing domain-category associations, allowing us to isolate the influence of spurious correlation shifts between ICE and test samples on MLLM generalization beyond other distribution shifts. 



==> paragraphs/impact.tex <==
\section*{Impact Statements}
\label{sect:impact}
This paper presents work whose goal is to advance the field of Machine Learning. There are many potential societal consequences of our work, none which we feel must be specifically highlighted here.
